Who's the (Multi-)Fairest of Them All: Rethinking Interpolation-Based Data Augmentation Through the Lens of Multicalibration

Data augmentation methods, especially SoTA interpolation-based methods such as Fair Mixup, have been widely shown to increase model fairness. However, this fairness is evaluated on metrics that do not capture model uncertainty and on datasets with only one, relatively large, minority group. As a remedy, multicalibration has been introduced to measure fairness while accommodating uncertainty and accounting for multiple minority groups. However, existing methods of improving multicalibration involve reducing initial training data to create a holdout set for post-processing, which is not ideal when minority training data is already sparse. This paper uses multicalibration to more rigorously examine data augmentation for classification fairness. We stress-test four versions of Fair Mixup on two structured data classification problems with up to 81 marginalized groups, evaluating multicalibration violations and balanced accuracy. We find that on nearly every experiment, Fair Mixup \textit{worsens} baseline performance and fairness, but the simple vanilla Mixup \textit{outperforms} both Fair Mixup and the baseline, especially when calibrating on small groups. \textit{Combining} vanilla Mixup with multicalibration post-processing, which enforces multicalibration through post-processing on a holdout set, further increases fairness.

==> sections/001_abstract.tex <==
\begin{abstract}
  % Existing data augmentation work measures algorithmic fairness with binary metrics that do not capture model uncertainty. However, methods of improving uncertainty-aware metrics involve reducing initial training data to create a holdout set for post-processing, which is not ideal when minority training data is already sparse. A promising direction in data augmentation for fairness is Fair Mixup, a variant of interpolation-based data augmentation that incorporates a fairness penalty between two computationally identifiable groups in its training loss. However, Fair Mixup has thus far been implemented on one relatively large minority group at a time, with performance reporting and training penalties based on binary demographic parity and equalized odds metrics. 
  
  % This paper uses multicalibration, which reflects probabilistic predictions, as an alternative lens to examine data augmentation for classification fairness. Using two structured data classification problems, we stress-test four versions of Fair Mixup with up to 81 marginalized groups, evaluating multicalibration violations and balanced accuracy against nine baselines, including post-processing, balanced batching, and regular mixup. We compare performance and fairness across five differently sized sets of demographic groups and 40 datasets per task. We surprisingly find that while Fair Mixup worsens performance and fairness in nearly all experiments, regular mixup substantially improves both, especially when calibrating on very small groups. Furthermore, combining regular mixup with multicalibration post-processing yields even stronger improvements than either procedure alone.

Data augmentation methods, especially SoTA interpolation-based methods such as Fair Mixup, have been widely shown to increase model fairness. However, this fairness is evaluated on metrics that do not capture model uncertainty and on datasets with only one, relatively large, minority group. As a remedy, multicalibration has been introduced to measure fairness while accommodating uncertainty and accounting for multiple minority groups. However, existing methods of improving multicalibration involve reducing initial training data to create a holdout set for post-processing, which is not ideal when minority training data is already sparse. This paper uses multicalibration to more rigorously examine data augmentation for classification fairness. We stress-test four versions of Fair Mixup on two structured data classification problems with up to 81 marginalized groups, evaluating multicalibration violations and balanced accuracy. We find that on nearly every experiment, Fair Mixup \textit{worsens} baseline performance and fairness, but the simple vanilla Mixup \textit{outperforms} both Fair Mixup and the baseline, especially when calibrating on small groups. \textit{Combining} vanilla Mixup with multicalibration post-processing, which enforces multicalibration through post-processing on a holdout set, further increases fairness.
\end{abstract}



==> sections/00_pretitle.tex <==
\usepackage[]{bibsty/aaai25}  % DO NOT CHANGE THIS
\usepackage{times}  % DO NOT CHANGE THIS
\usepackage{helvet}  % DO NOT CHANGE THIS
\usepackage{courier}  % DO NOT CHANGE THIS
\usepackage[hyphens]{url}  % DO NOT CHANGE THIS
\usepackage{graphicx} % DO NOT CHANGE THIS
\urlstyle{rm} % DO NOT CHANGE THIS
\def\UrlFont{\rm}  % DO NOT CHANGE THIS
\usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\usepackage{amsmath}
\usepackage{amssymb}
\frenchspacing  % DO NOT CHANGE THIS
\setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS
\setlength{\pdfpageheight}{11in} % DO NOT CHANGE THIS
%
% These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{booktabs}
\usepackage{xcolor}

%
% These are are recommended to typeset listings but not required. See the subsubsection on listing. Remove this block if you don't have listings in your paper.
\usepackage{newfloat}
\usepackage{listings}
\usepackage{xspace}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}
%
% Keep the \pdfinfo as shown here. There's no need
% for you to add the /Title and /Author tags.
\pdfinfo{
/TemplateVersion (2025.1)
}

% DISALLOWED PACKAGES
% \usepackage{authblk} -- This package is specifically forbidden
% \usepackage{balance} -- This package is specifically forbidden
% \usepackage{color (if used in text)
% \usepackage{CJK} -- This package is specifically forbidden
% \usepackage{float} -- This package is specifically forbidden
% \usepackage{flushend} -- This package is specifically forbidden
% \usepackage{fontenc} -- This package is specifically forbidden
% \usepackage{fullpage} -- This package is specifically forbidden
% \usepackage{geometry} -- This package is specifically forbidden
% \usepackage{grffile} -- This package is specifically forbidden
% \usepackage{hyperref} -- This package is specifically forbidden
% \usepackage{navigator} -- This package is specifically forbidden
% (or any other package that embeds links such as navigator or hyperref)
% \indentfirst} -- This package is specifically forbidden
% \layout} -- This package is specifically forbidden
% \multicol} -- This package is specifically forbidden
% \nameref} -- This package is specifically forbidden
% \usepackage{savetrees} -- This package is specifically forbidden
% \usepackage{setspace} -- This package is specifically forbidden
% \usepackage{stfloats} -- This package is specifically forbidden
% \usepackage{tabu} -- This package is specifically forbidden
% \usepackage{titlesec} -- This package is specifically forbidden
% \usepackage{tocbibind} -- This package is specifically forbidden
% \usepackage{ulem} -- This package is specifically forbidden
% \usepackage{wrapfig} -- This package is specifically forbidden
% DISALLOWED COMMANDS
% \nocopyright -- Your paper will not be published if you use this command
% \addtolength -- This command may not be used
% \balance -- This command may not be used
% \baselinestretch -- Your paper will not be published if you use this command
% \clearpage -- No page breaks of any kind may be used for the final version of your paper
% \columnsep -- This command may not be used
% \newpage -- No page breaks of any kind may be used for the final version of your paper
% \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% \pagestyle -- This command may not be used
% \tiny -- This is not an acceptable font size.
% \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

\setcounter{secnumdepth}{2} %May be changed to 1 or 2 if section numbers are desired.

\newcommand{\folktables}{\texttt{folktables}\xspace}

\newcommand{\base}{\textsc{Base}\xspace}
\newcommand{\fairbase}{\textsc{FairBase}\xspace}
\newcommand{\mpmc}{FM$_{\text{MC}}$\xspace}
\newcommand{\mpma}{FM$_{\text{MA}}$\xspace}
\newcommand{\fmeo}{FM$_{\text{EO}}$\xspace}
\newcommand{\fmdp}{FM$_{\text{DP}}$\xspace}
\newcommand{\enforcema}{\textsc{Enforce}$_{\text{MA}}$\xspace}
\newcommand{\enforcemc}{\textsc{Enforce}$_{\text{MC}}$\xspace}
\newcommand{\fairbaseeo}{\textsc{FairBase}$_{\text{EO}}$\xspace}
\newcommand{\fairbasema}{\textsc{FairBase}$_{\text{MA}}$\xspace}
\newcommand{\fairbasemc}{\textsc{FairBase}$_{\text{MC}}$\xspace}
\newcommand{\mixup}{\textsc{Mixup}\xspace}
\newcommand{\mixupeo}{\textsc{Mixup}$_{\text{EO}}$\xspace}
\newcommand{\mixupma}{\textsc{Mixup}$_{\text{MA}}$\xspace}
\newcommand{\mixupmc}{\textsc{Mixup}$_{\text{MC}}$\xspace}
\newcommand{\mixupenforcemc}{\textsc{Mixup$_{\textsc{Enforce}_{\text{MC}}}$}\xspace}

\newcommand{\all}{\textsc{All}\xspace}
\newcommand{\bigger}{\textsc{Big}\xspace}
\newcommand{\smaller}{\textsc{Small}\xspace}
\newcommand{\dis}{\textsc{Dis}\xspace}
\newcommand{\dislfr}{\textsc{DLFR}\xspace}

\newcommand{\employment}{\textsc{Employment}\xspace}
\newcommand{\income}{\textsc{Income}\xspace}

==> sections/00_title.tex <==
% Title

% Your title must be in mixed case, not sentence case.
% That means all verbs (including short verbs like be, is, using,and go),
% nouns, adverbs, adjectives should be capitalized, including both words in hyphenated terms, while
% articles, conjunctions, and prepositions are lower case unless they
% directly follow a colon or long dash
\title{Who's the (Multi-)Fairest of Them \all: Rethinking Interpolation-Based Data Augmentation Through the Lens of Multicalibration}
\author{
    %Authors
    % All authors must be in the same font size and format.
    Karina Halevy,\textsuperscript{\rm 1 2}
    Karly Hou,\textsuperscript{\rm 2}
    Charumathi Badrinath\textsuperscript{\rm 2}
}
\affiliations{
    %Afiliations
    \textsuperscript{\rm 1}Carnegie Mellon University\\
    \textsuperscript{\rm 2}Harvard University\\
    khalevy@andrew.cmu.edu
}




==> sections/01_introduction.tex <==
\begin{figure*}[th]
    \centering
    \includegraphics[width=0.9\linewidth,height=190px]{figs/pipeline.jpg}
    \caption{The ML training and evaluation pipelines considered in our work. Each method in our experiments can be characterized by a unique combination of: a percentage $p$ of post-processing data taken from training data, an interpolation-based data augmentation method $I$, a training batch selection procedure $S$, a training loss criterion $L$, a training fairness penalty $F$, and a post-processing algorithm $A$. These unique combinations are listed in Table \ref{tab:methods}.}
    \label{fig:fig1}
\end{figure*}
% equations: hard to visualize, maybe have a really toy example
% RQs: no mention of MA - cut that shit

Algorithmic fairness has become increasingly important with the ubiquitous application of machine learning (ML). Unfairness can arise from many sources \cite{Huang2022-oy}, including unequal representation of protected groups in data \cite{Guo2022-vx}. For example, people of color can be underrepresented in clinical trials due to access barriers, lack of information, and discrimination \cite{Allison2022-nv}, leading ML models to have trouble predicting treatment outcomes for non-white patients. One way to mitigate underrepresentation is data augmentation, which creates synthetic individuals from the original data \cite{chuang2021fair,iosifidisdealing,chawla2002smote,sharma2020idealworld}. A particularly promising form of augmentation is Mixup \cite{DBLP:journals/corr/abs-1710-09412} and its fairness-oriented counterpart Fair Mixup \cite{chuang2021fair}, which linearly interpolate individuals with features in between majority and minority group attributes. However, existing augmentation literature measures fairness through binary metrics like demographic parity and equalized odds \cite{chuang2021fair}, which accumulate loss even when predictors lean toward correct labels. These metrics can be misleading because data often does not include all predictive features, so some notion of uncertainty is appropriate in a good predictor but would be penalized. Furthermore, the methods in \citet{chuang2021fair} only assess and optimize fairness for one minority group, but a fair predictor should work well on multiple multi-dimensional intersecting groups.

The metric of multicalibration (MC) \cite{pmlr-v80-hebert-johnson18a} accounts for this uncertainty and for the presence of multiple groups by comparing predicted probabilities to true probabilities, averaging over groups of interest, and considering subsets of a predictor's support separately. \citet{pmlr-v80-hebert-johnson18a} also introduce an algorithm, with runtime inversely proportional to the size of the smallest group, to post-process a predictor using a holdout set and guarantee a maximum MC violation. \citet{covid_paper} then use this algorithm to learn prediction adjustments from a holdout set and apply those adjustments to test predictions. However, such post-processing subtracts a substantial amount of holdout data from available training data, resulting in even less representation of underrepresented groups in initial training. Moreover, with runtime inversely proportional to group size, enforcing MC for very small groups can be slow. The guarantees of MC enforcement and upper bounds of the overall accuracy tradeoffs proven in \citet{pmlr-v80-hebert-johnson18a} also only apply to the post-processed holdout set, not to unseen test data.

This work examines whether we can combine the desirable properties of MC and data augmentation. We ask:
\begin{enumerate}
    \item RQ1: Under what conditions can Fair Mixup mitigate MC violations of neural network predictors on minority groups while preserving binary classification accuracy?
    \item RQ2: When can (Fair) Mixup serve as an alternative to and/or increase the efficiency of MC post-processing?
    \item RQ3: What aspects of Fair Mixup contribute to its success or failure in improving MC-based fairness?
\end{enumerate}
We contribute the first MC-based investigation of several (Fair) Mixup- and MC-inspired neural network training methods (depicted in Figure \ref{fig:fig1}), stress-testing performance and fairness on intersecting demographic groups and creating a new perspective on whether data augmentation is effective. We find that Fair Mixup can only mitigate MC violations and outperform post-processing under its original design of optimizing one group at a time. However, vanilla Mixup consistently makes predictors fairer and results in an average balanced accuracy/MC violation improvement of up to 14.22\% when combined with MC post-processing. We also find that the key performance-enhancing component of Fair Mixup is that it learns from interpolated data points. However, its other components (balancing training data by minority group membership and penalizing pairwise unfairness during training) detract from baseline performance, resulting in average balanced accuracy/MC violation decreases of up to 12.29\%.

==> sections/02_preliminaries.tex <==
This section defines calibration \cite{pmlr-v80-hebert-johnson18a,chouldechova2017fair}, multicalibration \cite{pmlr-v80-hebert-johnson18a}, multiaccuracy \cite{pmlr-v80-hebert-johnson18a}, and  the data augmentation methods we later expand on. 
\subsection{Notation}
Throughout this paper, $\mathcal{X}$ represents a universe of individuals, $x_i$ represents an individual with index $i$, $S \subseteq \mathcal{X}$ is a subset of individuals, $\mathcal{C} \subseteq 2^{\mathcal{X}}$ is a set of subsets of individuals, $f$ is a predictor that maps individual $x_i$ to outcome probability $f_i$, $p_i^*$ is the true outcome probability of $x_i$, and $y_i \in \{0, 1\}$ is the binarized true outcome for $x_i$.
\subsection{Calibration}
For a maximum violation $\alpha \in [0,1]$, $f$ is $\alpha$\textbf{-calibrated} w.r.t. $S$ if $\exists S' \subseteq S$ with $|S'| \geq (1 - \alpha) |S|$ such that $\forall v \in [0,1],$
\begin{equation}\label{eq:calibration}
    |\mathbb{E}_{x_i \sim (S_v \cap S')}[f_i - p_i^*]| \leq \alpha,
\end{equation}
where $S_v = \{x_i:f_i = v\}$. In most classification tasks, we only see the binary outcome $y_i$ for $x_i$. Thus, we use a modification called \textbf{observable} calibration \cite{pmlr-v80-hebert-johnson18a}, where $y_i$ replaces $p_i^*$ in Eq. \ref{eq:calibration}.

For example, a tumor malignancy classifier is $0.05$-observably calibrated for $v = 0.6$ on Latine patients if of all Latine patients for which it predicts a 60\% chance of malignancy, 55\% to 65\% of these patients have a malignant tumor. The classifier is $0.05$-observably calibrated on Latine patients if this holds for all $v$---of all Latine patients for which it predicts a $v$ chance of malignancy, between $v - 5\%$ and $v + 5\%$ of these patients have a truly malignant tumor.

\subsection{Multicalibration}
$f$ is \textbf{$\mathbf{(\mathcal{C},\alpha)}$-multicalibrated} if it is $\alpha$-calibrated w.r.t. all $S \in \mathcal{C}$ \cite{pmlr-v80-hebert-johnson18a}. We define MC as in \citet{pmlr-v80-hebert-johnson18a}, but we require $S = S'$ (calibration on all of $S$ rather than any $1 - \alpha$ of it, explained in Appendix \ref{app:implementation}). For computational feasibility over datasets with millions of prediction probabilities, we also discretize the predicted probabilities. For integer $d > 0$, the $d$\textbf{-discretized} version of $S$ splits $S$ into $d + 1$ subsets, where
\begin{align}
    S_{v} = \{x_i: \frac{v}{d} \leq f_i < \frac{v + 1}{d}\} \text{ for } v \in [0,1,...,d].
\end{align}

Continuing with the tumor malignancy classifier example, the subset of the $10$-discretized $S = $ Latine patients with $v = 6$ would be all Latine patients with a predicted chance of at least $60\%$ but less than $70\%$ malignancy. Suppose all patients in this subset have a prediction of $63\%$. $0.05$-calibration would require that $58$ to $68\%$ of these patients have a truly malignant tumor, and that the corresponding conditions hold for all other $v \in [0, 10]$. Given $\mathcal{C} = \{$Black patients, Asian patients, Latine patients$\}$, $\mathcal{C}, 0.05$-multicalibration requires that this $0.05$-calibration must hold for Black, Asian, and Latine patients.
\subsection{Multiaccuracy}
Multiaccuracy (MA) \cite{pmlr-v80-hebert-johnson18a} is a looser version of MC. $f$ is $(\mathcal{C}, \alpha)$\textbf{-multiaccurate} if $ \forall S \in \mathcal{C}$,
\begin{equation}
    |\mathbb{E}_{x_i \sim S}[f_i - p_i^*]| \leq \alpha.
    \end{equation}
Rather than requiring the expected prediction error within each $S$ \textit{and} predicted probability to be $\leq \alpha$, MA only requires this error to be $\leq \alpha$ in $S$ overall. Thus, for $\mathcal{C}$ = $\{$Black patients, Latine patients$\}$, $(\mathcal{C}, 0.05)$-multiaccuracy means that the average prediction for Black patients is within 5\% of the true proportion of Black patients that have a malignant tumor, and likewise for Latine patients. In the rest of this paper, when we say $f$ has an MC or MA violation of $\alpha$ on $\mathcal{C}$, we mean that $\alpha$ is the smallest value for which $f$ is $(\mathcal{C}, \alpha)$-multicalibrated or multiaccurate.
\subsection{Mixup}\label{sec:mixup}
Mixup was proposed to improve the generalizability of neural networks (NN) by training on linear combinations of example pairs, with the intuition that the NN would learn how predictions differ as inputs move continuously between feature sets \cite{DBLP:journals/corr/abs-1710-09412}. For training batch size $b$, mixup draws $(x_1,y_1) ,...,(x_b, y_b)$ and $(x_1', y_1'),...,(x_b', y_b')$ without replacement from the training data. Let $t \sim \text{Beta}(\epsilon, \epsilon)$ where $\epsilon \in (0, \infty)$. Mixup constructs one synthetic point per $i \in [1, ..., b]$:
\begin{align}
    (x_i'',y_i'') = (t x_i + (1 - t)x_i', ty_i + (1 - t)y_i')
\end{align}
and trains an NN on $(x_1'', y_1''), \cdots, (x_b'', y_b'')$ instead of the original batch. \citet{DBLP:journals/corr/abs-1710-09412} showed that mixup decreased test error on CIFAR-10 and CIFAR-100.
\subsection{Fair Mixup}
\citet{chuang2021fair} adapted mixup toward the goal of fairness. \textbf{Fair Mixup} (FM) samples $(x_1,y_1) ,...,(x_b, y_b)$ from minority group $S$ and $(x_1', y_1'),...,(x_b', y_b')$ from $S' = \neg S$. Mixup is then performed on these samples as in Section \ref{sec:mixup} to create synthetic points. The loss function applies the standard Binary Cross Entropy (BCE) loss function to the original points, applies the gradient $\mathcal{R}_{\text{mixup}}^{\mathcal{M}_S}$ of a pairwise fairness penalty $\mathcal{M}$ between $S$ and $S'$ to the synthetic points, and adds $\lambda$ times the fairness penalty to the BCE. Fair Mixup creates better tradeoffs between average precision and the fairness metrics of demographic parity and equalized odds \cite{chuang2021fair}.



==> sections/03_relatedwork.tex <==
\subsection{Data Augmentation for Fairness}
There are several other data augmentation methods for fairness. In oversampling, minority group samples are duplicated until equal in number to majority group samples \cite{iosifidisdealing}. Another method, SMOTE, creates minority group members through linear interpolation among existing minority group members \cite{chawla2002smote}. More recently, \citet{sharma2020idealworld} introduce ``Ideal World'': for each original point, a new sample is created with the same features and label, but the protected attribute is flipped, making both statistical parity difference and average odds difference decrease while preserving accuracy. Outside of structured data, \citet{Wadhwa} apply identity pair replacement, identity term blindness, and identity pair swap on text classification. \citet{dur30710} introduce data augmentation that improves facial recognition on minority groups.

We focus on structured data classification to minimize the confounding factor of unstructured data featurization. We also choose Fair Mixup as a basis because it minimizes data distribution changes and treats protected attributes as predictive features. Ideal World takes away the predictive information of protected attributes. Oversampling, SMOTE, and Ideal World create additional minority individuals, changing the frequency and composition of minority groups. In contrast, Fair Mixup creates individuals that are neither minority nor majority group members, but rather some interpolated in-between. Thus, while the data distribution may change, the members of boolean circuit-defined groups do not.

\subsection{Extensions of MC}
\citet{pmlr-v80-hebert-johnson18a} devise algorithms that could enforce MC $\alpha$'s to be below an arbitrary threshold. A related post-processing algorithm, designed for multiaccuracy, is \textsc{Multiaccuracy Boost}, which requires a trained auditor on top of a holdout set \cite{kim2019multiaccuracy}. Applying the results of \citet{pmlr-v80-hebert-johnson18a} empirically, \citet{covid_paper} transfer learned post-processing updates to a COVID-19 mortality rate forecasting task. We test this application in Section \ref{subsubsec:pp}. 

A few works extend (multi-)calibration to more nuanced metrics that handle complex notions of uncertainty. \citet{pmlr-v80-kumar18a} add calibration optimization to the training loss function, clamping overconfident predictions while minimizing penalties on true confident predictions. \citet{wald2021on} propose multi-domain calibration to evaluate model generalization to out-of-distribution data, suggesting both isotonic regression post-processing and a training regime that includes calibration from \citet{pmlr-v80-kumar18a}. \citet{pmlr-v134-jung21a} extend MC to higher moments, measuring moment consistency in a way that computes groupwise error inversely proportionally to group size \cite{pmlr-v134-jung21a}. Other work extends MC to conformal prediction, which generates prediction sets rather than point estimates \cite{jung2023batch,barber2020limits}. This framework generalizes MC to quantiles of the label's support rather than individual values and is useful for categorical or continuous labels, unlike binary labels, for which MC is already a probabilistic extension. \citet{omnipredictors-for-regression} connect MC to multi-group loss minimization.

The most comprehensive investigation of MC post-processing to our knowledge is \citet{hansen2024multicalibrationpostprocessingnecessary}, which finds that baseline predictors on tabular data are often decently multicalibrated already, and post-processing does not improve worst-group calibration error for multi-layer perceptrons, Random Forests, and Logistic Regression but does benefit Support Vector Machines, Decision Trees, and Naive Bayes. When worst-group calibration error improves, there is an overall accuracy tradeoff. They further find that MC enforcement is hyperparameter-sensitive and most effective with huge amounts of data (found in image and language data but not tabular data). They find that calibration algorithms like Platt scaling and isotonic regression sometimes perform nearly on par with MC enforcement while being more efficient. These findings are consistent with previous works suggesting that empirical risk minimization may inevitably yield multicalibrated baseline predictors \cite{blasiok2023when,blasiok2024loss}. We refer the reader to \citet{hansen2024multicalibrationpostprocessingnecessary} for a more comprehensive MC literature review and for image and language experiments.

This work extends \citet{hansen2024multicalibrationpostprocessingnecessary} in three ways. First, expanding upon their maximum of 15 groups that are all at least 0.5\% of their corresponding population, we stress-test our methods on MC w.r.t. up to 81 groups at a time, up to 55 of which are smaller than 0.25\% of their corresponding population. We also select these groups in five different ways to investigate effects of group set size on MC. Second, expanding upon their examination of income prediction from \texttt{folktables} on Californian residents from 2018, we evaluate our methods on each permutation of the 10 most populous US states and the four most recent American Community Survey data collection years, yielding 40 datasets. We additionally test employment status prediction on these 40 datasets, for a total of 80 tasks considered. Third, while their work and much of the current MC literature considers data-reductive post-processing methods, our work takes inspiration from their finding that post-processing works best on huge datasets and instead focuses on data augmentation to maximize the amount of original data that can be used for initial training.

==> sections/04_methods.tex <==
\begin{table*}[th]\fontsize{9pt}{9pt}\selectfont
    \centering
    \begin{tabular}{c|ccp{2.8cm}ccc}\toprule
      Method   &  $p$ & $I$ & $S$ & $L$ & $F$ & $A$  \\\midrule
       \base  & 0 & $I(\cdot) = []$ & uniform random & BCE & $F(\cdot) = 0$ & $A(\cdot) = []$\\
       \fairbase & 0 & $I(\cdot) = []$ & balance by group & BCE & $F(\cdot) = 0$ & $A(\cdot) = []$\\
       \mixup & 0 & Mixup & uniform random & $L(\cdot) = 0$ & BCE & $A(\cdot) = []$ \\
       \mixupeo & 0 & Mixup & balance by group $\times y_i$  & BCE & $\lambda \cdot \text{BCE}$ & $A(\cdot) = []$ \\
       \mixupma & 0 & Mixup & balance by group & BCE & $\lambda \cdot \text{BCE}$ & $A(\cdot) = []$ \\
       \mixupmc & 0 & Mixup & balance by group $\times f_i$ & BCE & $\lambda \cdot \text{BCE}$ & $A(\cdot) = []$ \\
       \fmdp & 0 & Mixup & balance by group  & BCE & $\lambda \cdot \mathcal{R}_{\text{mixup}}^{\text{DP}}$ & $A(\cdot) = []$ \\
       \fmeo & 0 & Mixup & balance by group $\times y_i$ & BCE & $\lambda \cdot \mathcal{R}_{\text{mixup}}^{\text{EO}}$ & $A(\cdot) = []$ \\
       \mpma & 0 & Mixup & balance by group & BCE & $\lambda \cdot \mathcal{R}_{\text{mixup}}^{\text{MA}}$ & $A(\cdot) = []$ \\
       \mpmc & 0 & Mixup & balance by group $\times f_i$ & BCE & $\lambda \cdot \mathcal{R}_{\text{mixup}}^{\text{MC}}$ & $A(\cdot) = []$ \\
       \enforcema & 25 & $I(\cdot) = []$ & uniform random & BCE & $F(\cdot) = 0$ & Listing \ref{lst:ma}\\
       \enforcemc & 25 & $I(\cdot) = []$ & uniform random & BCE & $F(\cdot) = 0$ & Listing \ref{lst:mc}\\
       \mixupenforcemc & 25 & Mixup & uniform random & $L(\cdot) = 0$ & BCE & Listing \ref{lst:mc} \\
         \bottomrule
    \end{tabular}
    \caption{Post-processing data split percentages $p$, data augmentors $I$, training batch selectors $S$, loss criteria $L$ (applied to original data), fairness penalties $F$ (applied to synthetic data), and post-processing algorithms $A$ that uniquely characterize each method described in Section \ref{sec:methods} and diagrammed in Fig. \ref{fig:fig1}. BCE stands for Binary Cross Entropy loss.}
    \label{tab:methods}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=0.93\linewidth,height=140px]{figs/methods.jpg}
    \caption{Venn Diagram of each method's core components.}
    \label{fig:methods}
\end{figure}
We test 13 NN training methods to determine the effects of particular features of FM that contribute to its performance and fairness. FM has 3 distinguishing components: \begin{enumerate}
    \item C1: Training batches are balanced across membership in the minority group for which we wish to ensure fairness.
    \item C2: Synthetic data is created by linearly interpolating original points. If C1 is implemented, each synthetic data point is the interpolation of a minority group member and a majority group member. If not, the original points are split in half and paired at random for interpolation.
    \item C3 (can only be done if C2 is also implemented): A fairness penalty is added to the loss function for predictions on synthetic points, minimizing a weighted sum of the standard loss and the fairness penalty during training.
\end{enumerate}
Post-processing is distinguished by the following: \begin{enumerate}\setcounter{enumi}{3}
    \item C4: A post-processing algorithm learns prediction update rules from post-processing data (subtracted from initial training data), and it applies those update rules to the validation and test data during evaluation and deployment.
\end{enumerate}
With these insights (summarized in Fig. \ref{fig:methods}), this section describes each method mathematically. We motivate each method by explaining how it implements a subset of $\{$C1, C2, C3, C4$\}$, thus isolating the effects of specific components of FM to answer RQ3. C4 also helps answer RQ2 (FM vs{.} post-processing). Method names are starred if they contain substantial novel elements that we introduce on top of existing work. Implementation details are in Appendix \ref{app:implementation}.
\subsection{Baselines}
\subsubsection{\base} trains an NN with mini-batch gradient descent using Binary Cross Entropy loss, over several epochs and batch selection iteration. We report test-time balanced accuracy for the epoch with the best validation-time balanced accuracy. \base does not implement C1, C2, C3, or C4.
\subsubsection{$^*$\fairbase} modifies \base by balancing training data groupwise (C1). Suppose we have minority groups $\mathcal{C}$ to optimize for fairness and $n$ iterations of gradient descent per training epoch in \base. Then, \fairbase conducts $n \cdot |\mathcal{C}|$ iterations of gradient descent. Each iteration centers around one $S \in \mathcal{C}$: we construct a batch by selecting one sub-batch from $S$ and one sub-batch from its complement $\neg S$. We subsample the larger sub-batch to be equal in size to the smaller sub-batch to ensure balance across membership in $S$.
\subsection{Variants of Mixup}
\subsubsection{\mixup} is as defined in Section \ref{sec:mixup}, implementing C2.
\subsubsection{$^*$\mixupeo} modifies \fairbase. Consider minority groups $\mathcal{C}$ and $n \cdot |\mathcal{C}|$ iterations of gradient descent as in \fairbase. \mixupeo conducts $2n \cdot |\mathcal{C}|$ iterations of gradient descent, each centered around one pair $(S, y) \in (\mathcal{C}, \{0, 1\})$. We construct a batch by selecting one sub-batch of members of $S_y$ (members of $S$ whose true label is $y$) and one sub-batch of members of $S'_y$ (members of $\neg S$ whose true label is $y$). Next, we perform mixup by pairing each member of $S_y$ with a member of $S'_y$ within the batch and interpolating each pair. Our loss is a weighted sum of Binary Cross Entropy applied to the original batch and the same loss applied to the interpolated points. \mixupeo implements C1, C2, and a control version of C3 (standard loss instead of pairwise fairness, but number of groups under consideration for this loss is adjustable, as elaborated on in Section \ref{subsubsec:fmmod}). Thus, we can compare it to \fairbase to isolate the effect of C2.
\subsubsection{$^*$\mixupma} creates one balanced batch per $S \in \mathcal{C}$, as in \fairbase, yielding $n \cdot |\mathcal{C}|$ gradient descent iterations. We interpolate each batch by pairing members of $S$ with members of $\neg S$ and adding $\lambda$ times the Binary Cross Entropy on the interpolated points. \mixupma also implements C1, C2, and a control version of C3, though C1 is slightly different than in \mixupeo, allowing us to compare variations of C1.
\subsubsection{$^*$\mixupmc} creates $d + 1$ batches per $S \in \mathcal{C}$ by creating $d$-discretized intervals of $f_i$'s, yielding $(d + 1) \cdot n \cdot |\mathcal{C}|$ gradient descent iterations. For each $S_v^d$ (members of $S$ with predicted probability in $[\frac{v}{d}, \frac{v + 1}{d})$), we construct a batch with half its points from members of $S_v$ and the other half from members of $(\neg S)_v^d$. 
We interpolate and calculate loss as in \mixupeo. \mixupmc also implements C1, C2, and a control version of C3, providing another way to compare the specifics of C1.

\subsection{Variants of Fair Mixup}\label{subsec:fm}
FM implements C1, C2, and C3. Though \citet{chuang2021fair} introduce two versions of FM (with $\mathcal{M}$ as demographic parity difference and equalized odds difference), their framework generalizes to any pairwise fairness metric. We first show how to modify FM to accommodate multiple minority groups simultaneously. Then, we define the two versions of FM from \citet{chuang2021fair}, followed by two versions with new metrics. Specifically, our extensions try to incorporate some notion of MC in the fairness penalty, as we aim to minimize MC violations. These methods test the effects of varying the metric in C3.
\subsubsection{Modifying (Fair) Mixup for Multiple Groups}\label{subsubsec:fmmod}
Consider metric $\mathcal{M}$, its group gradients $ \mathcal{R}_{\text{mixup}}^{\mathcal{M}_{S_1}},..., \mathcal{R}_{\text{mixup}}^{\mathcal{M}_{S_{|\mathcal{C}|}}}.$
For $k \in \{1,...,|\mathcal{C}|\}$, the penalty is the mean of the $k$ highest group gradients. We take means because preliminary experiments show that sums produce higher MC $\alpha$s. We make $k$ adjustable to prevent overfitting. The rest of the computation proceeds as in \citet{chuang2021fair}. Given $\mathcal{M}_S$, the first step is to transform it into an integral via the Fundamental Theorem of Calculus so it can be computed for interpolated data (Appendix A.1 in \citet{chuang2021fair}). Then, we differentiate the integral to get $\mathcal{R}_{\text{mixup}}^{\mathcal{M}_{S}}$. We list the equations for $\mathcal{M}_S$ below, with full formulae in Appendix \ref{app:fm}. 
\subsubsection{\fmdp} is the first version of FM in \citet{chuang2021fair}. $\mathcal{M}_S$ is demographic parity, the difference between the average $f_i$ on members of $S$ vs{.} its complement $S'$: \begin{equation}
    \mathcal{M}_S = \Delta \text{DP}_S(f) \\
    = |\mathbb{E}_{x_i \sim S}[f_i] - \mathbb{E}_{x_i \sim S'}[f_i]|.
\end{equation} 
\subsubsection{\fmeo} is the second version of FM, with the equalized odds difference \cite{hardt2016equality} that modifies DP by only considering one true outcome at a time: \begin{equation}
    \mathcal{M}_S = \Delta \text{EO}_{S}(f) \\
    = \sum_{y \in \{0, 1\}}|\mathbb{E}_{x_i \sim S_y}[f_i] - \mathbb{E}_{x_i \sim S'_y}[f_i]|,
\end{equation} where $S_y = \{x_i \in S: y_i = y\}$, and $S' = \neg S$. 
\subsubsection{$^*$\mpma} is our first extension of FM, with a version of MA modified to be pairwise. We measure the mean difference in prediction errors $e_i = f_i - p_i^*$ between $S$ and $S'$:
\begin{equation}
    \mathcal{M}_S = \Delta \text{MA}_S(f) \\
    = |\mathbb{E}_{x_i \sim S}[e_i] - \mathbb{E}_{x_i \sim S'}[e_i]|,
\end{equation} 
\subsubsection{$^*$\mpmc} is our second extension of FM, with a pairwise modification of MC, which modifies MA by considering one interval $S_{v}^d = \{ x_i \in S: f_i \in [\frac{v}{d}, \frac{v + 1}{d}) \}$ at a time:
\begin{equation}
    \mathcal{M}_S = \Delta \text{MC}_S(f) = \sum_{v = 0}^d |\mathbb{E}_{x_i \sim S_{v}^d}[e_i] - \mathbb{E}_{x_i \sim S'^d_{v}}[e_i]|.
\end{equation} 

\subsection{Post-Processing}\label{subsubsec:pp}
We test whether MC and MA enforcement (implementing C4) improve test performance as in \citet{covid_paper}.
\subsubsection{\enforcema} post-processes predictions to minimize MA violations. We feed (1) predictions on a holdout post-processing set and (2) a set of minority groups $\mathcal{C}$ as inputs to Algorithm 3.1 in \citet{pmlr-v80-hebert-johnson18a}. However, we augment Algorithm 3.1 with a list of rules mapping each $S \in \mathcal{C}$ to a float $a_S$ to be added to predictions on members of $S$. In other words, the algorithm learns how much to adjust predictions for each group. At validation and test time, we add $a_S$ to initial predictor outputs for members $S$.
\subsubsection{\enforcemc} post-processes predictions to minimize MC violations. It proceeds as in \enforcema, but we add an integer $d$ as a third input to Algorithm 3.2 in \citet{pmlr-v80-hebert-johnson18a}. We augment Algorithm 3.2 with a list of rules mapping each group $S_v$ (members of $S \in \mathcal{C}$ where $f_i \in [\frac{v}{d}, \frac{v + 1}{d})$), to a float $a_{S, v}$ to be added to predictions on members of $S$ whose initial predictions are in $[\frac{v}{d}, \frac{v + 1}{d})$.
\subsubsection{\mixupenforcemc} performs \mixup on a reduced initial training set followed by \enforcemc on a holdout post-processing set. This method tests C2 $\cup$ C4, as we ultimately find that \mixup performs best overall among methods that do not implement C4. We implement \mixupenforcemc to answer the part of RQ2 that asks whether data augmentation can improve the performance of \enforcemc.

==> sections/05_experiments.tex <==
This section describes our data and experimental settings.

\subsection{Datasets}
\begin{table*}[ht]\fontsize{9pt}{9pt}\selectfont
    \centering
    \begin{tabular}{ccp{2.3cm}ccp{1.4cm}p{1.8cm}p{1.75cm}}\toprule
     Dataset & Size & \# Features (Binary, Categorical, Continuous) & \# Non-White  & \# Disabled & Max \# Minority Groups  & Max \# Groups $\leq$ 0.25\% of Population & Mean Size of Smallest Group \\\midrule
    \employment & 6,993,839 & 5, 9, 2 & 2,160,161 & 1,036,251 & 81 & 55 & 28.5 \\
    \income    & 3,543,292 & 2, 3, 6 & 1,014,632 & 250,074 & 51 & 28 & 31.85\\
         \bottomrule
    \end{tabular}
     \caption{Summary statistics of the \employment and \income datasets. ``Size'' is the number of individuals summed over all 40 subsets. Maxes and means are taken over these subsets. ``Smallest Group'' disabled members of the LFR.}
    \label{tab:data_stats}
\end{table*}
We test two prediction tasks from \folktables \cite{ding2021retiring}, a superset of Adult Income data \cite{KohaviBecker} collected from the American Community Survey. We have $p_i^* \in \{0, 1\}$, but $f_i \in [0, 1]$. Table \ref{tab:data_stats} summarizes the data. Full data statistics are at \url{http://tiny.cc/mfm-stats}.

\paragraph{\employment} The task is to predict whether an individual is employed. Table \ref{tab:employment_features} specifies the exact input features.

\paragraph{\income} The task is to predict whether an individual's annual income is higher than the median income for that year in their state of residence according to Data Commons \cite{datacommons}. Table \ref{tab:income_features} lists input features.

We run 40 datasets each for \employment and \income: the 10 most populous US states $\times$ the 4 most recent years. We choose these tasks based on experiments in \citet{jung2023batch}. Additionally, we seek problems with reasonable baseline performance ($\geq 80\%$ balanced accuracy on CA $\times$ 2022) to focus on improving fairness on useful classifiers.
\subsection{Experimental Settings}
To measure the effects of $|\mathcal{C}|$ and $|S|$, we run all combinations of datasets and training methods on five settings:

\subsubsection{\all} $\mathcal{C} = \cup$ $\{$all $n$ computationally possible racial groups, disabled people, disabled members of each racial group$\}$. A racial group is computationally possible if for all random seeds, at least one disabled member of that group is in each of the train, validation, and test splits. $|\mathcal{C}| = \mathbf{2n + 1}$.
\subsubsection{\bigger} $\mathcal{C} = \cup$ \{$b$ racial groups each comprising $>$ 0.25\% of the total dataset, disabled people, disabled members of each of the $b$ racial groups.$\}$ $|\mathcal{C}| = \mathbf{2b + 1}, \mathbf{b << n}$.
\subsubsection{\smaller} $\mathcal{C} = \cup$ $\{s$ racial groups each comprising $\leq$ 0.25\% of the total dataset, disabled people, disabled members of each of the $s$ racial groups$\}$. $|\mathcal{C}| = \mathbf{2s + 1}, \mathbf{s << n}$.
\subsubsection{\dis} This setting is closest to what FM has already been tested on: $\mathcal{C} = \{\text{disabled individuals}\}$, so $|\mathcal{C}| = \mathbf{1}$.
\subsubsection{\dislfr} $\mathcal{C} = $ disabled people, members of the least frequent (computationally possible) racial group (LFR), and disabled members of the LFR, hence $|\mathcal{C}| = \mathbf{3}$.






==> sections/06_results.tex <==
\begin{table*}[ht]\fontsize{9pt}{9pt}\selectfont
\setlength{\tabcolsep}{1mm}
\centering
  \begin{tabular}{p{2.5cm}|ccccc|ccccc}\toprule
Method &  & &\employment & & &  &  & \income &  \\
 &  \all & \bigger & \smaller & \dis & \dislfr & \all & \bigger & \smaller & \dis & \dislfr \\\midrule
 \base &	0.00	&	0.00	&	0.00	&	0.00	&	0.00	&	0.00	&	0.00	&	0.00	&	0.00	&	0.00 \\
    \fairbase & -2.69	&	-2.36	&	-4.28	&	2.08	&	-3.76	&	-3.04	&	-4.26	&	-11.08	&	-12.29	&	-6.34 \\
     \mixup &	2.89	&	3.11	&	2.56	&	-23.20	&	2.03	&	1.22	&	1.30	&	\textbf{3.12}	&	\textbf{3.20}	&	1.63	 \\
   \mixupeo &	-2.54	&	-2.21	&	-4.66	&	4.45	&	-4.07	&	-3.39	&	-4.14	&	-9.73	&	-12.09	&	-6.15 \\
   \mixupma &	-3.31	&	-3.08	&	-4.70	&	\textbf{4.50}	&	-5.35	&	-3.10	&	-3.51	&	-11.51	&	-10.80	&	-7.27 \\
    \mixupmc &	-2.91	&	-2.55	&	-5.30	&	3.09	&	-5.93	&	-3.08	&	-3.02	&	-10.34	&	-10.78	&	-6.58 \\ 
    \fmdp &	-3.41	&	-2.22	&	-5.23	&	3.84	&	-5.29	&	-3.34	&	-3.39	&	-10.75	&	-10.11	&	-7.67 \\
    \fmeo &	-2.26	&	-3.36	&	-4.05	&	1.73	&	-4.52	&	-3.55	&	-3.58	&	-10.00	&	-11.12	&	-5.55 \\
    \mpma &	-2.95	&	-3.99	&	-6.35	&	1.40	&	-5.79	&	-3.74	&	-3.41	&	-10.33	&	-11.92	&	-7.36 \\
    \mpmc &	-2.72	&	-2.36	&	-4.94	&	0.61	&	-4.12	&	-4.32	&	-3.23	&	-10.41	&	-11.30	&	-5.52 \\
     \enforcema &	-0.46	&	0.02	&	0.46	&	0.43	&	-0.32	&	-0.02	&	0.70	&	-1.27	&	-2.76	&	-1.66 \\
    \enforcemc  &	8.31	&	12.03	&	7.89	&	-15.28	&	\textbf{8.74}	&	9.87	&	9.97	&	-6.61	&	-17.82	&	8.28 \\
    \mixupenforcemc 	&	\textbf{10.36}	&	\textbf{12.97}	&	\textbf{9.23}	&	-29.27	&	8.72	&	\textbf{11.64}	&	\textbf{14.22}	&	-2.15	&	-11.37	&	\textbf{13.06} \\
    \bottomrule
\end{tabular}
\caption{Summary (mean of 10 trials) of methods across 40 (state, year) pairs $\times$ \employment and \income. Each number is the mean of the \% increase in balanced accuracy and \% decrease in worst-group MC $\alpha$.}
\label{tab:result_summary}
\end{table*}

To capture both fairness and overall performance, we compute the mean across all 40 (state, year) pairs of the following quantities for each experiment: (1) \% increase in balanced accuracy over \base for the corresponding state, year, and task and (2) \% decrease over \base in worst (highest) individual group MC violation $\alpha$. 
Table \ref{tab:result_summary} reports these mean percentages, showing that for all (task, setting) pairs except for \dis (both tasks), (\employment, \dislfr), and (\income, \smaller), \mixupenforcemc shows the biggest average balanced accuracy and MC $\alpha$ improvement. 
The other best methods are \mixupma for (\employment, \dis), \mixup for (\income, \dis) and (\income, \smaller), \enforcemc for (\employment, \dislfr) (though \mixupenforcemc is close), but \fmdp has the best $\alpha$ for (\employment, \dis) according to Table \ref{tab:worst_mc_summary}. If we consider only methods that perform post-processing or augmentation/data balancing (i.e. all methods except \mixupenforcemc), the best method is \enforcemc, except (\employment, \dis) (\mixupma was best), (\income, \smaller), and (\income, \dis) (\mixup was best). One note is that for 28 of 40 datasets, we had $s = 0$ and thus $\mathcal{C} = $ just disabled people, so (\income, \smaller) results may be more characteristic of single-group calibration. We also note that all methods except for \base had negative mean increases in balanced accuracy (up to -1.25\%), so positive values in Table \ref{tab:result_summary} indicate fairness improvements.

Examining FM, we see that except (\employment, \dis), all FM variants worsened fairness. For (\employment, \dis), FM improved fairness while largely preserving balanced accuracy, confirming the result in \citet{chuang2021fair} that FM works on one larger group. 

Comparing \mixupenforcemc and \enforcemc, we observe that while \mixupenforcemc outperforms \enforcemc in many cases, it sometimes makes the \enforcemc component of \mixupenforcemc less efficient. On the \employment dataset, the number of iterations to convergence of the \enforcemc post-processing algorithm increased by a percentage in the range $(0.34\%, 5.8\%)$, with the greatest percentage increase for \smaller (+5.8\%) and the greatest decrease for \bigger (-1.58\%). For \income, all methods took fewer iterations, in the range $(-3.68\%, -0.08\%)$. 

Finally, we analyze correlations between results and data statistics. We largely find either no correlation or low correlations, with some exceptions. One exception is that the mean MC $\alpha$ across groups $> 0.25\%$ of the population on \all has a moderate correlation with total dataset size (lower violations for bigger datasets) for all non-\base methods that do not involve \enforcemc. This mean $\alpha$ on \all also moderately correlates with the number of groups bigger than $0.25\%$ of the population for \mpma, and it also moderately correlates with number of groups smaller than $0.25\%$, total number of minority groups, number of disabled individuals, and number of non-white individuals for several methods. Looking at efficiency, the number of iterations to convergence of \enforcemc and \mixupenforcemc both strongly correlate with dataset size, but there is no correlation with the \% change in number of iterations between methods.


==> sections/07_Discussion.tex <==
Our results reveal the importance of stress-testing fairness optimization on multiple groups of varying sizes and on metrics that capture uncertainty. To answer RQ1, \textbf{the only condition under which FM improves MC is the condition it was designed for}: fairness for one minority group (\dis) on a truly binary problem (\employment). This holds irrespective of the particular train-time fairness penalty. This leads to an answer to RQ2: under a \textbf{single-group truly-binary condition}, FM (especially \fmdp) outperforms post-processing in ensuring fairness for disabled people. Based on the raw $\alpha$s in Table \ref{tab:worst_mc_summary}, this could be because disabled people are a relatively big, non-monolithic group for which the \base NN is already much more calibrated than the more fine-grained racial groups. Thus, to further improve upon the \base $\alpha$, it may be more effective to examine more disabled individuals and their full feature sets during training (as in FM) rather than apply a fixed adjustment to disabled individuals unconditionally (as in post-processing). However, this fixed post-processing adjustment may work well for smaller racial groups because the smaller sizes of racial groups make race more informative than disability.

\textbf{Regular \mixup presents a robust alternative} to \enforcema in nearly all settings and to \enforcemc when considering one group in a continuous-to-binary prediction problem as in (\income, \dis) or part of (\income, \smaller). More powerfully, \textbf{combining \mixup and \enforcemc through \mixupenforcemc enhances performance} of \enforcemc alone in the majority of settings, especially when more than one group is under consideration. However, it is inconclusive whether this enhancement is accompanied by efficiency improvement for the \enforcemc component.

For RQ3, we see that \textbf{\mixup is the overall best post-processing-free method}. Comparing \mixup with \mixupeo, \mixupma, \mixupmc, and \fairbase, we observe that \textbf{using interpolated data contributes more to fairness improvements} than groupwise balancing of training batches. Looking at \fairbase, \mixupeo, \mixupma, and \mixupmc, we further suggest that \textbf{data balancing may adversely affect performance and fairness}. Finally, comparing \mixupeo, \mixupma, and \mixupmc to FM variants, we see that C3 effects (train-time fairness penalty) are inconclusive, as outcomes fluctuate by method and setting.

==> sections/08_conclusion.tex <==
We conduct the first investigation of how data augmentation via interpolation affects MC-based fairness on multiple minority groups of multiple sizes for binary tabular data classification. We find that while Fair Mixup is not so fair on multiple groups, regular mixup mitigates MC violations across many groups, both by itself and together with MC post-processing. Our investigation opens several avenues of future work on effects of data augmentation on probabilistic fairness in other modalities (e.g. vision, language) and ML problems (e.g. continuous/categorical labels).

==> sections/09_ethics.tex <==
Augmentation introduces synthetic data and alters demographic representation to present the illusion that certain groups are well-represented. We urge creators and users of augmented datasets to be transparent about augmentation methods used. We lead by example as we release our datasets with full methodological descriptions.

==> sections/10_acks.tex <==
We thank Professor Cynthia Dwork and Pranay Tankala for teaching the course that inspired this work and for mentoring us through the initial stages of the project. We also thank Professor Maarten Sap and Alfredo Gomez for helpful feedback during the paper writing and rebuttal process.
